Nutzungsverhalten und Funktionsanforderungen digitaler Trainingsanwendungen w\"ahrend der Pandemie

Due to contact restrictions, closure of fitness centers and quarantine measures, the SARS-CoV-2 pandemic led to a considerable decline of sporting activities. The first relaxation of these restrictions allowed German citizens to mostly return to their normal training and exercise behavior, yet the long-term impact of the recurring measures (i.e. the "Lockdown", "Lockdown light" as well as the "Corona Emergency Break" in the case of Germany) remain rather under-investigated. Using a survey of (n=108) German sportspersons, we measured a significant decline of sporting activities even within the intermediary phases without major pandemic constraints. To evaluate the capabilities of digital training applications in countering these effects, we additionally recorded the usage of, among others, apps, trackers, videos and conferencing systems and identified the most important as well as missing and/or essential features with regards to their capabilities of facilitating individual sport and training in times without access to facilities or social contacts. Effectively, the usage of smart watches, online videos and conferences increased significantly when compared to before the pandemic; and especially online videos and conferences contributed to higher training frequencies. Data-driven or individual feedback, motivation and collaboration revealed to be the most important or even necessary functions for users of digital training applications to counter the decline of social components of training.

==> copypastestuff.tex <==

% \begin{table}[h]
% \begin{center}
% \begin{minipage}{174pt}
% \caption{Caption text}\label{tab1}%
% \begin{tabular}{@{}llll@{}}
% \toprule
% Column 1 & Column 2  & Column 3 & Column 4\\
% \midrule
% row 1    & data 1   & data 2  & data 3  \\
% row 2    & data 4   & data 5\footnotemark[1]  & data 6  \\
% row 3    & data 7   & data 8  & data 9\footnotemark[2]  \\
% \botrule
% \end{tabular}
% \footnotetext{Source: This is an example of table footnote. This is an example of table footnote.}
% \footnotetext[1]{Example for a first table footnote. This is an example of table footnote.}
% \footnotetext[2]{Example for a second table footnote. This is an example of table footnote.}
% \end{minipage}
% \end{center}
% \end{table}

% \begin{table}[h]
% \begin{center}
% \begin{minipage}{\textwidth}
% \caption{Example of a lengthy table which is set to full textwidth}\label{tab2}
% \begin{tabular*}{\textwidth}{@{\extracolsep{\fill}}lcccccc@{\extracolsep{\fill}}}
% \toprule%
% & \multicolumn{3}{@{}c@{}}{Element 1\footnotemark[1]} & \multicolumn{3}{@{}c@{}}{Element 2\footnotemark[2]} \\\cmidrule{2-4}\cmidrule{5-7}%
% Project & Energy & $\sigma_{calc}$ & $\sigma_{expt}$ & Energy & $\sigma_{calc}$ & $\sigma_{expt}$ \\
% \midrule
% Element 3  & 990 A & 1168 & $1547\pm12$ & 780 A & 1166 & $1239\pm100$\\
% Element 4  & 500 A & 961  & $922\pm10$  & 900 A & 1268 & $1092\pm40$\\
% \botrule
% \end{tabular*}
% \footnotetext{Note: This is an example of table footnote. This is an example of table footnote this is an example of table footnote this is an example of~table footnote this is an example of table footnote.}
% \footnotetext[1]{Example for a first table footnote.}
% \footnotetext[2]{Example for a second table footnote.}
% \end{minipage}
% \end{center}
% \end{table}

% \begin{sidewaystable}
% \sidewaystablefn%
% \begin{center}
% \begin{minipage}{\textheight}
% \caption{Tables which are too long to fit, should be written using the ``sidewaystable'' environment as shown here}\label{tab3}
% \begin{tabular*}{\textheight}{@{\extracolsep{\fill}}lcccccc@{\extracolsep{\fill}}}
% \toprule%
% & \multicolumn{3}{@{}c@{}}{Element 1\footnotemark[1]}& \multicolumn{3}{@{}c@{}}{Element\footnotemark[2]} \\\cmidrule{2-4}\cmidrule{5-7}%
% Projectile & Energy	& $\sigma_{calc}$ & $\sigma_{expt}$ & Energy & $\sigma_{calc}$ & $\sigma_{expt}$ \\
% \midrule
% Element 3 & 990 A & 1168 & $1547\pm12$ & 780 A & 1166 & $1239\pm100$ \\
% Element 4 & 500 A & 961  & $922\pm10$  & 900 A & 1268 & $1092\pm40$ \\
% Element 5 & 990 A & 1168 & $1547\pm12$ & 780 A & 1166 & $1239\pm100$ \\
% Element 6 & 500 A & 961  & $922\pm10$  & 900 A & 1268 & $1092\pm40$ \\
% \botrule
% \end{tabular*}
% \footnotetext{Note: This is an example of table footnote this is an example of table footnote this is an example of table footnote this is an example of~table footnote this is an example of table footnote.}
% \footnotetext[1]{This is an example of table footnote.}
% \end{minipage}
% \end{center}
% \end{sidewaystable}

% \begin{figure}[h]%
% \centering
% \includegraphics[width=0.9\textwidth]{fig.eps}
% \caption{This is a widefig. This is an example of long caption this is an example of long caption  this is an example of long caption this is an example of long caption}\label{fig1}
% \end{figure}
